DiffuseGAE: Controllable and High-fidelity Image Manipulation from Disentangled Representation

Diffusion probabilistic models (DPMs) have shown remarkable results on various image synthesis tasks such as text-to-image generation and image inpainting. However, compared to other generative methods like VAEs and GANs, DPMs lack a low-dimensional, interpretable, and well-decoupled latent code. Recently, diffusion autoencoders (Diff-AE) were proposed to explore the potential of DPMs for representation learning via autoencoding. Diff-AE provides an accessible latent space that exhibits remarkable interpretability, allowing us to manipulate image attributes based on latent codes from the space. However, previous works are not generic as they only operated on a few limited attributes. To further explore the latent space of Diff-AE and achieve a generic editing pipeline, we proposed a module called Group-supervised AutoEncoder(dubbed GAE) for Diff-AE to achieve better disentanglement on the latent code. Our proposed GAE has trained via an attribute-swap strategy to acquire the latent codes for multi-attribute image manipulation based on examples. We empirically demonstrate that our method enables multiple-attributes manipulation and achieves convincing sample quality and attribute alignments, while significantly reducing computational requirements compared to pixel-based approaches for representational decoupling. Code will be released soon.

==> figures/mlp_and_bottleneck.tex <==
\begin{figure}[htb]
\centering
% \vspace{-10pt}
\setlength{\abovecaptionskip}{-0.5pt}
\includegraphics[width=1\linewidth]{figures/images/mlp_and_bottleneck.pdf}
\caption{GROUP$(z_c, 1)$ of~$z_{sem} ~\text{dataset} ~\mathcal{D}_z$ on ilab\_20M. We adopt supervised attribute-swap and unsupervised attribute-swap to further disentangle ~$z_{sem}$ obtained from diffusion autoencoders in an autoencoding manner. In our paper, ~$z_{sem}(decoupled)$ is equivalent to ~$z_{dis}$ 
Our Group AutoEncoder(GAE) is a common encoder-decoder architecture.}
\label{fig:group_overview}
\vspace{-10pt}
\end{figure}

==> hyphen.tex <==
\hyphenation{sinusoi-dal ac-cepts acc-epts Trans-former Co-FiNet CoFi-Net sce-narios scena-rios domi-nated Al-though Alth-ough gene-rate genera-te hie-rarchical em-bedding Geo-metric gene-rates}



\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\argmin}{\arg\!\min} 



\def\secname#1{\textcolor{red}{#1}}
\def\head#1{\noindent\textbf{#1}}
\def\tight#1{\hspace{1pt}{#1}{\hspace{1pt}}}
\def\medium#1{\hspace{2pt}{#1}{\hspace{2pt}}}
\def\wide#1{\hspace{3pt}{#1}{\hspace{3pt}}}
\newcommand{\slfrac}[2]{\left.#1\middle/#2\right.}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newlength{\wdth}
\newcommand{\strike}[1]{\settowidth{\wdth}{#1}\rlap{\rule[.5ex]{\wdth}{.4pt}}#1}
\newcommand{\ptitle}[1]{\noindent\textbf{#1}\hspace{5pt}}
% \newcommand\notsotiny{\@setfontsize\notsotiny{6}{7}}

\newcommand{\kx}[1]{{\color{red}#1}}
\newcommand{\tofix}[1]{{\color{red}[Fix: #1]}}
\newcommand{\num}{{\color{blue}[X]~}}
\newcommand{\supl}[1]{{\color{black}\emph{#1}}}
\newcommand{\fix}[1]{{\color{blue}#1}}
